Inter-Layer Scheduling Space Exploration for Multi-model Inference on Heterogeneous Chiplets

To address increasing compute demand from recent multi-model workloads with heavy models like large language models, we propose to deploy heterogeneous chiplet-based multi-chip module (MCM)-based accelerators. We develop an advanced scheduling framework for heterogeneous MCM accelerators that comprehensively consider complex heterogeneity and inter-chiplet pipelining. Our experiments using our framework on GPT-2 and ResNet-50 models on a 4-chiplet system have shown upto 2.2x and 1.9x increase in throughput and energy efficiency, compared to a monolithic accelerator with an optimized output-stationary dataflow.

==> Tables/eval_results.tex <==

\begin{table}[t]
    \centering
    \caption{Evaluation of the two-stage pipelined GPT-2 and ResNet-50 for a batch size of 1, input sizes of 128$\times$1 and 224$\times$224$\times$3 Bytes.}
    \vspace{-2ex}
    \begin{tabular}{l | c c | c c}
    \hline
    \multirow{2}{*}{Model} & \multicolumn{2}{c|}{GPT-2} & \multicolumn{2}{c}{ResNet-50} \\ 
    & stage I & stage II & stage I & stage II \\ \cline{1-5}
    EDP-os (kJ.s) & 127.4 & 239.0 & 9.8 & 23.3 \\
    EDP-ws (kJ.s) & 511.9 & 955.0 & 4.6 & 7.6 \\ \hline
    latency-os (ms) & 456.4 & 907.0 & 34.6 & 55.1 \\
    latency-ws (ms)  & 1966.4 & 3627.6 & 82.1 & 80.1 \\ \hline
    Interchiplet Traffic & \multicolumn{2}{c|}{96 KBs} & \multicolumn{2}{c}{392 KBs} \\ \cline{1-5}
    
    %   latency-os & 0.33.5 & 66.5 & 38.5 & 61.5 \\
    % latency-ws & 35.2 & 64.8 & 50.6 & 49.4 \\ \hline  
    % \multirow{2}{*}{ResNet50} & mAP & 28.8 & \textbf{29.9} & \textbf{27.1}  \\
    % & Lat. (ms) & 122.06 & \textbf{98.84} & \textbf{78.96} \\
    % \cline{1-5}
    % \multirow{2}{*}{ResNet18} & mAP & 27.3 & \textbf{26.8} & \textbf{26.3}  \\
    % & Lat. (ms) & 55.99 & \textbf{42.21} & \textbf{31.38} \\
    % \cline{1-5}
    \end{tabular}
    \label{tab:models}
    \vspace{-4ex}
\end{table}


